Spike-and-Slab Posterior Sampling in High Dimensions

Posterior sampling with the spike-and-slab prior [MB88], a popular multimodal distribution used to model uncertainty in variable selection, is considered the theoretical gold standard method for Bayesian sparse linear regression [CPS09, Roc18]. However, designing provable algorithms for performing this sampling task is notoriously challenging. Existing posterior samplers for Bayesian sparse variable selection tasks either require strong assumptions about the signal-to-noise ratio (SNR) [YWJ16], only work when the measurement count grows at least linearly in the dimension [MW24], or rely on heuristic approximations to the posterior. We give the first provable algorithms for spike-and-slab posterior sampling that apply for any SNR, and use a measurement count sublinear in the problem dimension. Concretely, assume we are given a measurement matrix $\mathbf{X} \in \mathbb{R}^{n\times d}$ and noisy observations $\mathbf{y} = \mathbf{X}\mathbf{\theta}^\star + \mathbf{\xi}$ of a signal $\mathbf{\theta}^\star$ drawn from a spike-and-slab prior $\pi$ with a Gaussian diffuse density and expected sparsity k, where $\mathbf{\xi} \sim \mathcal{N}(\mathbb{0}_n, \sigma^2\mathbf{I}_n)$. We give a polynomial-time high-accuracy sampler for the posterior $\pi(\cdot \mid \mathbf{X}, \mathbf{y})$, for any SNR $\sigma^{-1}$ > 0, as long as $n \geq k^3 \cdot \text{polylog}(d)$ and $X$ is drawn from a matrix ensemble satisfying the restricted isometry property. We further give a sampler that runs in near-linear time $\approx nd$ in the same setting, as long as $n \geq k^5 \cdot \text{polylog}(d)$. To demonstrate the flexibility of our framework, we extend our result to spike-and-slab posterior sampling with Laplace diffuse densities, achieving similar guarantees when $\sigma = O(\frac{1}{k})$ is bounded.

==> tex_file/mean_estimation.tex <==
%!TEX root = ../root.tex

\section{Simple Case study: Mean Estimation}
\subsection{Core Term of Posterior}
In this section, we assume $X$ is the identity matrix and assume 
\begin{equation}
    y = \theta + \epsilon,
\end{equation}
where $y, \theta, \epsilon \in \bbR^{d}$, $\epsilon \sim \calN(0_d, \sigma^2 I_d)$. 
In this case the posterior degenerates into 
\begin{align}
    \pi(S|y) &= \frac{\pi(y, S)}{\pi(y)}= \frac{1}{\pi(y)}\int_{\Omega_\theta} \pi(y, \theta, S)\diff\theta \nonumber\\
    &= \frac{1}{\pi(y)}\int_{\Omega_\theta} \pi(y|\theta, S) \pi(\theta|S)\pi_0(S)\diff\theta \nonumber\\
    &= \frac{1}{\pi(y)}\int_{\Omega_\theta} \pi(y|\theta) \pi(\theta|S)\pi_0(S)\diff\theta \nonumber\\
    \label{eq:post_1_mean_est}
    &\propto q^{|S|}(1 - q)^{d-|S|}\int_{\Omega_{\theta_S}}\exp\paren{-\frac{1}{2\sigma^2}\twonorm{y - (\theta_S, 0)}^2 - \frac{1}{2}\twonorm{\theta_S}^2}\diff \theta_S,
\end{align}
where we let $(\theta_S, 0)$ to reserve only the coordinates in $S$ of $\theta$ and set all other coordinates to be zero. 

Then we consider the second order term: 
\begin{align*}
    &-\frac{1}{2\sigma^2}\twonorm{y - (\theta_S, 0)}^2 - \frac{1}{2}\twonorm{\theta_S}^2\\
    =& -\frac{1}{2}\paren{\frac{1 + \sigma^2}{\sigma^2}\twonorm{\theta_S}^2 - 2\frac{1}{\sigma^2}\theta_S^\top y_S + \frac{\twonorm{y}^2}{\sigma^2}}\\
    =& -\frac{\twonorm{y}^2}{2\sigma^2} + \frac{1}{2}\frac{\twonorm{y_S}^2}{\sigma^2(1+\sigma^2)} - \frac{1+\sigma^2}{2\sigma^2} \twonorm{ \theta_S - \frac{y}{1+\sigma^2}}^2.
\end{align*}
Inserting it back to Eq. \ref{eq:post_1_mean_est}, we have 
\begin{align*}
    \pi(S|y) &\propto q^{|S|}(1-q)^{d-|S|}\exp\paren{\frac{\twonorm{y_S}^2}{2\sigma^2(1+\sigma^2)}}\int_{\Omega_\theta}\exp \paren{-\frac{1+\sigma^2}{2\sigma^2}}\twonorm{ \theta_S - \frac{y_S}{1+\sigma^2}}^2 \\
    &\propto \paren{\frac{k}{d-k}\sqrt{\frac{2\pi\sigma^2}{1+\sigma^2}}}^{|S|}\exp\paren{\frac{\twonorm{y_S}^2}{2\sigma^2(1+\sigma^2)}}.
\end{align*}

\subsection{Experiment with Gaussian Prior.}
In this case, we first have 
\begin{align*}
    \pi(S|y) &= \frac{1}{\pi(y)}\int_{\Omega_\theta} \pi(y|\theta) \pi(\theta|S)\pi_0(S)\diff\theta\\
    &\propto q^{|S|}(1 - q)^{d-|S|}\int_{\Omega_{\theta_S}}\exp\paren{-\frac{1}{2\sigma^2}\twonorm{y - (\theta_S, 0)}^2 - \frac{1}{2}\twonorm{\theta_S}^2}\diff \theta_S
\end{align*}
Then we consider the second order term: 
\begin{align*}
    -\frac{1}{2\sigma^2}\twonorm{y - (\theta_S, 0)}^2 - \frac{1}{2}\twonorm{\theta_S}^2
    &= -\frac{1}{2}\paren{\frac{1 + \sigma^2}{\sigma^2}\twonorm{\theta_S}^2 - 2\frac{1}{\sigma^2}\theta_S^\top y_S + \frac{\twonorm{y}^2}{\sigma^2}}\\
    &= -\frac{\twonorm{y}^2}{2\sigma^2} + \frac{1}{2}\frac{\twonorm{y_S}^2}{\sigma^2(1+\sigma^2)} - \frac{1+\sigma^2}{2\sigma^2} \twonorm{ \theta_S - \frac{y}{1+\sigma^2}}^2 
\end{align*}
Inserting it back, we have 
\begin{align*}
    \pi(S|y) &\propto q^{|S|}(1-q)^{d-|S|}\exp\paren{\frac{\twonorm{y_S}^2}{2\sigma^2(1+\sigma^2)}}\int_{\Omega_\theta}\exp \paren{-\frac{1+\sigma^2}{2\sigma^2}}\twonorm{ \theta_S - \frac{y_S}{1+\sigma^2}}^2 \\
    &\propto \paren{\frac{q}{1 - q}\sqrt{\frac{2\pi\sigma^2}{1+\sigma^2}}}^{|S|}\exp\paren{\frac{\twonorm{y_S}^2}{2\sigma^2(1+\sigma^2)}}\\
    &= \prod_{i \in S}\paren{\frac{q}{1 - q}\sqrt{\frac{2\pi\sigma^2}{1 + \sigma^2}} \exp \paren{\frac{y_i^2}{2\sigma^2(1+\sigma^2)}}}
\end{align*}

We first provide an algorithm for sampling a support set, $\tilde{S} \sim \tpi\paren{.|y,X}$ below -
\begin{algorithm}[H]
    \caption{post sample with Gaussian prior in mean est case$\left(y, \sigma^{2}, q\right)$}
    \label{alg:post_sample}
    \KwIn{Observed Data $D := \left\{X \in \bbR^{n \times d}, y \in \bbR^{n}\right\}$, Noise variance $\sigma^{2}$, Prior Selection Probability $q \in \paren{0,1}$}
    \KwOut{Sampled Support Set $\tilde{S} \sim \tpi\paren{.|y,X}$}
    Initialize $\tilde{S} \leftarrow \left\{\right\}$ 
    
    Let $\forall i \in [d],$ let $ p_{i} \leftarrow \prod_{i \in S}\paren{\sqrt{\frac{2\pi\sigma^2}{1 + \sigma^2}} \exp \paren{\frac{y_i^2}{2\sigma^2(1+\sigma^2)}}}$     
    
    \For{$i \in [d]$}{
        Sample
        \bas{
            \xi_{i} := \begin{cases}
                1 \text{ with probability } \frac{qp_{i}}{1 - q + qp_{i}} \\
                0 \text{ otherwise }
            \end{cases}
        }
        Include $i$ in $\tilde{S}$ if $\xi_{i} = 1$
    }
    \Return $\tilde{S}$
\end{algorithm}
